3D-FM GAN: Towards 3D-Controllable Face Manipulation

3D-controllable portrait synthesis has significantly advanced, thanks to breakthroughs in generative adversarial networks (GANs). However, it is still challenging to manipulate existing face images with precise 3D control. While concatenating GAN inversion and a 3D-aware, noise-to-image GAN is a straight-forward solution, it is inefficient and may lead to noticeable drop in editing quality. To fill this gap, we propose 3D-FM GAN, a novel conditional GAN framework designed specifically for 3D-controllable face manipulation, and does not require any tuning after the end-to-end learning phase. By carefully encoding both the input face image and a physically-based rendering of 3D edits into a StyleGAN's latent spaces, our image generator provides high-quality, identity-preserved, 3D-controllable face manipulation. To effectively learn such novel framework, we develop two essential training strategies and a novel multiplicative co-modulation architecture that improves significantly upon naive schemes. With extensive evaluations, we show that our method outperforms the prior arts on various tasks, with better editability, stronger identity preservation, and higher photo-realism. In addition, we demonstrate a better generalizability of our design on large pose editing and out-of-domain images.

==> Table/SOTA_comparison.tex <==
\begin{table}[t]
    \fontsize{9}{10}\selectfont
    
    \centering
    \begin{tabular}{|c|c|c|c|c|c|}
    \hline
     & Vari~\cite{buhler2021varitex} & CON~\cite{kowalski2020config} & Lift~\cite{shi2021lifting} & DisCo~\cite{deng2020disentangled} & Ours \\
     \hline
     FID$^{\downarrow}$ & 34.4 &  33.4 & 29.8 & 19.7 & \textbf{12.2} \\
    \hline
     
    \end{tabular}
    \caption{Photo realism comparison against state of the arts. 
    Our method achieves the best performance.  }
    \label{tab:SOTA_comparison}
\end{table}

==> limitation.tex <==
\section{Limitations \& Negative Societal Impacts}

Although \Ours\ shows a strong ability for 3D-controllable identity-preserved face editing, 
there remains certain limitations and potential negative impacts. 

\noindent\textbf{Limitations.} Our 3DMMs can not model fine details like wrinkles and hair styles,
and thus our model can not explicitly control those attributes.
We also see a gap between the reconstructed images and the inputs in face shapes, which might be caused by the imprecise 3D estimation in face reconstruction.
Moreover, our model would inherit bias from the training data, and due to lack of public availability,
we can only use synthetic data for disentangled learning.

\noindent\textbf{Potential Negative Impacts.}
Face manipulation techniques has in the past helped creating deep-fakes and spread disinformation. Our work is intended for intelligent content creation for portrait photography and we believe it does not improve the accessibility of deep-fakes and disinformation. Moreover, our discoveries of identity-editability trade-off might also offer new viewpoints on future development for deep-fake detection techniques.


% The main motivation of our method is to enable intelligent content creation for portrait photography, yet it might be used to generate deep-fakes for disinformation. However, it neither improves the accessibility of deep-fakes, nor makes them harder to detect. Moreover, we believe research development in deep-fake detection models will mitigate this issue in the future. 

